Ev-TTA: Test-Time Adaptation for Event-Based Object Recognition

We introduce Ev-TTA, a simple, effective test-time adaptation algorithm for event-based object recognition. While event cameras are proposed to provide measurements of scenes with fast motions or drastic illumination changes, many existing event-based recognition algorithms suffer from performance deterioration under extreme conditions due to significant domain shifts. Ev-TTA mitigates the severe domain gaps by fine-tuning the pre-trained classifiers during the test phase using loss functions inspired by the spatio-temporal characteristics of events. Since the event data is a temporal stream of measurements, our loss function enforces similar predictions for adjacent events to quickly adapt to the changed environment online. Also, we utilize the spatial correlations between two polarities of events to handle noise under extreme illumination, where different polarities of events exhibit distinctive noise distributions. Ev-TTA demonstrates a large amount of performance gain on a wide range of event-based object recognition tasks without extensive additional training. Our formulation can be successfully applied regardless of input representations and further extended into regression tasks. We expect Ev-TTA to provide the key technique to deploy event-based vision algorithms in challenging real-world applications where significant domain shift is inevitable.

==> 3_method.tex <==
\section{Method}
\label{sec:method}

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of label collapse occuring due to training the entire network.}
   \label{fig:optim}
\end{figure}

Ev-TTA adapts a pre-trained event classifier $F_\theta(\cdot)$ with parameters $\theta$ trained on the source domain to a target domain.
The source domain is defined as the original external condition used for training and the target domain is similarly defined as the new condition used for testing.
Ev-TTA aims to resolve large domain gaps such as training on ambient lighting and testing on low lighting.

Event classifiers predict class probabilities using the event camera output $\mathcal{E}=\{e_i=(x_i, y_i, t_i, p_i)\}$, where $e_i$ indicates brightness change with polarity $p_i \in \{-1, 1\}$ at pixel location $(x_i, y_i)$ at time $t_i$.
Event classification algorithms often employ a two-step procedure, where events are first aggregated to form an image-like representation, and further processed using a classifier to output class probabilities.
While there are several approaches that directly process events~\cite{eventnet, asynet, snn}, we retain our focus on classifiers that employ image-like event representations.

Ev-TTA operates by optimizing the training objective that imposes temporal consistency (Section~\ref{sec:objective}), where the input event representation is conditionally refined using spatial consistency (Section~\ref{sec:noise}).

\begin{figure}[t!]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.95\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Overview of Training Objective.}
   \label{fig:overview}
\end{figure}

\paragraph{Test-Time Adaptation Strategy}
Following Tent~\cite{tent}, we choose to only optimize the batch normalization layers of the pre-trained classifier.
This design choice is crucial for Ev-TTA to properly function.
Figure~\ref{fig:optim} shows the t-SNE visualization of the 3-way classification results on one of the N-ImageNet~\cite{n_imagenet} variants recorded under extreme camera motion.
Even using the identical objective, training the entire network results in the predicted labels to collapse, leading to worse results in the target domain.
As the classifier parameters $\theta$ contain crucial priors about event camera data, altering the entire set of parameters may divert the model from its training~\cite{tent}.
Therefore, we constrain the optimization to only operate on the batch normalization parameters.
The total training loss $\mathcal{L}$ is optimized only once for each training sample in the target domain.
Nonetheless, Ev-TTA can successfully perform adaptation.

Ev-TTA is evaluated either in an offline or online manner.
In the offline setup, Ev-TTA is first optimized for the entire target domain, and subsequently performs another set of inference for evaluation using the same samples with the updated model parameters.
In the online setup, Ev-TTA is simultaneously evaluated and optimized, thus omitting the second inference phase.
Ev-TTA shows strong performance in both evaluation scenarios, where the detailed results are reported in Section~\ref{sec:exp}.
Note that no data from the source domain is used again for training, which would lead to large amounts of additional computation as source domain data is typically much larger than the target domain.
Further, no modifications in the neural network architecture or the training process is required, thus enlarging the applicability of Ev-TTA.


\subsection{Training Objective}
\label{sec:objective}
As shown in Figure~\ref{fig:overview}, Ev-TTA minimizes the loss function defined as $\mathcal{L}=\mathcal{L}_{\text{pred}}+\mathcal{L}_{\text{cond}}$, where $\mathcal{L}_{\text{pred}}$ is the prediction similarity loss and $\mathcal{L}_{\text{cond}}$ is the conditional entropy loss.
Both losses utilize the temporal aspects of the event data by imposing consistency in the time domain.

\paragraph{Prediction Similarity Loss}
Given an event stream $\mathcal{E}$, let $\mathcal{E}_\text{1}, \dots, \mathcal{E}_\text{K} \subset \mathcal{E}$ be the K random slices of equal length obtained from $\mathcal{E}$.
For event-based object recognition the input events span no more than 100ms, and thus we can assume the K random event slices to be temporally adjacent.
Prediction similarity loss enforces the predicted label distributions for the temporally neighboring events $\mathcal{E}_1, \dots, \mathcal{E}_K$ to be similar.

Using the symmetric KL divergence $S_{\text{KL}}(P, Q) = D_{\text{KL}}(P \| Q) + D_{\text{KL}}(Q \| P)$, prediction similarity loss is defined as follows,
\begin{equation}
\label{eq:sim}
    \mathcal{L}_{\text{pred}}= \frac{1}{2} \sum_{k=2}^{K} S_{\text{KL}}(F_\theta(\mathcal{E}_1), F_\theta(\mathcal{E}_k)),
\end{equation}
where $F_\theta(\cdot)$ is the event classifier with parameters $\theta$.
Note that the loss minimizes the discrepancy between the prediction for the first event slice and the rest.
Conceptually, label prediction for the first event slice acts as an anchor that pulls the predictions of other event slices.
While the formulation could be extended to incorporate all possible pairs within the K event slices, this would lead to a quadratic increase in computation.
A comparison using only a single event slice as an anchor is sufficient for successful adaptation. 
We also find that the choice of the anchor does not have a significant effect on performance, where an in-depth analysis is deferred to the supplementary material.

\paragraph{Selective Entropy Loss}
While the prediction similarity loss provides a meaningful learning signal for test-time adaptation, it is not sufficient for successful adaptation.
Since the loss heavily depends on the quality of the anchor prediction, it is important to enforce the anchor to make valid predictions in the target domain.
To this end, Ev-TTA leverages an selective entropy loss to the predictions on the first event slice $\mathcal{E}_\text{1} \subset \mathcal{E}$, namely the anchor.

Inspired from SENTRY~\cite{sentry}, we propose to selectively minimize the prediction entropy only if the anchor event slice $\mathcal{E}_\text{1}$ is consistent.
This is determined by examining whether the predicted class labels are in agreement with the temporally neighboring events.
To elaborate, each event slice $\mathcal{E}_\text{i}$ casts a vote on the class label with the highest probability, namely $v_\text{i} = \argmax F_\theta(\mathcal{E}_\text{i})$.
An anchor is considered consistent if its label vote $v_1$ is equal to the majority vote from the other event slices $\mathcal{V}_{\text{other}}=\{v_\text{2}, \dots, v_\text{K}\}$.
Using the entropy $H(p)=-\sum_\text{i} p_\text{i} \log p_\text{i}$ defined for a discrete probability distribution $p \in \mathbb{R}^{\text{C}}$ where C is number of classes, selective entropy loss is defined as follows,

\begin{equation}
    \mathcal{L}_{\text{cond}} = 
\left\{
	\begin{array}{ll}
		H(F_\theta(\mathcal{E}_\text{1}))  & \mbox{if consistent} \\
		0 & \mbox{if inconsistent.}
	\end{array}
\right.
\label{eq:select}
\end{equation}

Note that our loss formulation differs from the selective entropy loss of SENTRY~\cite{sentry} in two ways.
First, the criterion for consistency is determined using temporally neighboring events, unlike the image  augmentations used in SENTRY.
Further, while SENTRY~\cite{sentry} proposes to maximize the predicted entropy for samples that are inconsistent, we find that simply ignoring these samples as in Equation~\ref{eq:select} is more effective for test-time adaptation in event vision.
We further validate this claim in the ablation study from Section~\ref{exp:abl}.

\paragraph{Extension to Regression}

Our loss formulation can be easily extended to other task setups as long as the output is a probability distribution.
We demonstrate that Ev-TTA could be utilized for regression, which together with classification constitute a large portion of computer vision tasks.

Event-based steering angle prediction is a regression task where the object is to predict the steering angle $\phi$ from a stream of events $\mathcal{E}$.
To accommodate the formulation of Ev-TTA, we design the regressor to predict both the mean and variance of the steering angle, namely $F_\theta(\mathcal{E}) = (\mu, \sigma)$.
Assuming that the output variables follow a Gaussian distribution, the regressor is trained to maximize the log likelihood as in Nix \etal~\cite{gauss},
\begin{equation}
    \mathcal{L}_\text{likelihood}=-\log \sigma - \frac{(\phi_\text{gt} - \mu)^2}{2\sigma^2},
\end{equation}
where $\phi_\text{gt}$ is the ground-truth steering angle from the source domain.

Under such conditions we make several modifications to the loss functions used in Ev-TTA for classification. 
We first replace the symmetric KL divergence from Equation~\ref{eq:sim} using the KL divergence of Gaussian distributions, namely
\begin{equation}
    S_\text{KL}(F_\theta(\mathcal{E}_1), F_\theta(\mathcal{E}_\text{k})) = 
    \frac{\sigma_1^4 + \sigma_\text{k}^4 + (\sigma_1^2+\sigma_\text{k}^2)(\mu_1 - \mu_\text{k})^2}{2\sigma_1^2\sigma_\text{k}^2}.
\end{equation}
We also alter the entropy from Equation~\ref{eq:select} with the entropy of Gaussian distributions, namely
\begin{equation}
    H(F_\theta(\mathcal{E}_\text{1})) = \log \sigma_1 \sqrt{2\pi\text{e}}.
\end{equation}
Finally, the consistency criterion is modified for continuous network outputs.
An anchor event is considered consistent if its predicted variance is within a range of variances predicted from its neighbors.
To elaborate, we verify if the ratio of variances $\sigma_1^2 / \sigma_\text{k}^2$ for $k=\text{2},\dots, \text{K}$ is bounded within $10^{-1}$ and $10$.
We impose constraints using the variance since the predicted mean may deviate largely depending on the driving scenario, whereas the predicted variance should be consistent over a longer time horizon.
Together, the three major alterations in Ev-TTA lead to performance enhancements in steering angle prediction, which is further discussed in Section~\ref{exp:perf}.

\begin{figure}[t!]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.95\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Illustration of noise removal.}
   \label{fig:noise}
\end{figure}


\subsection{Conditional Noise Removal}
\label{sec:noise}

We propose to conditionally remove noise in low-light conditions using a criterion derived from the spatial consistency of events.
In low-light conditions, a sudden burst of noise in a single polarity may occur, as shown in Figure~\ref{fig:change}.
This occurs due to the "dark currents"~\cite{v2e} that constantly flow through the phototransistors gaining strength in low light where the currents for valid events become smaller.
Such noise can cause large amounts of performance deterioration in low-light settings, as noted from Kim \etal~\cite{n_imagenet}.

To alleviate performance degradation, we perform conditional noise removal on the anchor event $\mathcal{E}_1$ from Section~\ref{sec:objective}.
The noise removal operation only takes place if there is a large imbalance in the ratio of positive and negative events.
To determine whether the noise burst has occurred, we perform statistical hypothesis testing using the ratio distribution of events.
Let $N_\text{pos}, N_\text{neg}$ denote the number of pixels containing positive and negative events, respectively.
Assuming $N_\text{pos}, N_\text{neg}$ follow a Gaussian distribution, the following transformation to the ratio $R=N_\text{pos} / N_\text{neg}$ follows a standard Gaussian distribution~\cite{cond_rat},
\begin{equation}
    T(R) = \frac{\mu_\text{neg}R - \mu_\text{pos}}{\sqrt{\sigma_\text{pos}^2R^2-2\rho\sigma_\text{pos}\sigma_\text{neg}R+\sigma_\text{neg}^2R^2}},
\end{equation}
where $\mu_\text{pos}, \mu_\text{neg}$ is the mean, $\sigma_\text{pos}, \sigma_\text{neg}$ is the standard deviation, and $\rho$ is the cross-correlation of $N_\text{pos}, N_\text{neg}$.

Using the events from the source domain, we obtain the statistics $\{\mu_\text{pos}, \mu_\text{neg}, \sigma_\text{pos}, \sigma_\text{neg}, \rho\}$.
If an event stream from the target domain does not contain a noise burst, we can expect the transformed event ratio $T(R)$ using the source domain statistics to follow a standard Gaussian distribution.
Given a batch of anchor events from the target domain, we compute the transformed ratios and apply statistical hypothesis testing to determine if the batch is in accord with the source domain. 
Further details about the hypothesis testing procedure is deferred to the supplementary material.

Depending on the hypothesis test, if a batch contains significant polarity imbalance we perform noise removal using spatial consistency.
We illustrate the noise removal operation using a two-channel event representation $P=\{P_\text{pos}, P_\text{neg}\} \in \mathbb{R}^{H \times W \times 2}$, where $P_\text{pos}, P_\text{neg}$ are the positive and negative channels respectively.
As shown in Figure~\ref{fig:noise}, we denoise the channel with noise burst (in this case $P_\text{pos}$) if a pixel containing events lack spatial neighbors in the opposite polarity.
The modified channel $\Tilde{P}_\text{pos}$ replaces the original channel to form a new anchor event representation $\Tilde{P}=\{\Tilde{P}_\text{pos}, P_\text{neg}\}$, which is further used to compute the losses defined in Equation~\ref{eq:sim},~\ref{eq:select}.
Note that our noise removal method mainly targets noise burst in low light, unlike existing denoising mechanisms~\cite{denoise_exp_special, density_filter, ev_gait} which consider a much broader set of noise.
Nevertheless, our method is extremely light-weight as it could be implemented with simple masking and effectively removes noise burst, which we demonstrate in Section~\ref{exp:abl}.

